Analysing Mechanisms for Virtual Channel Management in Low-Diameter networks

To interconnect their growing number of servers, current supercomputers and data centers are starting to adopt low-diameter networks, such as HyperX, Dragonfly and Dragonfly+. These emergent topologies require balancing the load over their links and finding suitable non-minimal routing mechanisms for them becomes particularly challenging. The Valiant load balancing scheme is a very popular choice for non-minimal routing. Evolved adaptive routing mechanisms implemented in real systems are based on this Valiant scheme. All these low-diameter networks are deadlock-prone when non-minimal routing is employed. Routing deadlocks occur when packets cannot progress due to cyclic dependencies. Therefore, developing efficient deadlock-free packet routing mechanisms is critical for the progress of these emergent networks. The routing function includes the routing algorithm for path selection and the buffers management policy that dictates how packets allocate the buffers of the switches on their paths. For the same routing algorithm, a different buffer management mechanism can lead to a very different performance. Moreover, certain mechanisms considered efficient for avoiding deadlocks, may still suffer from hard to pinpoint instabilities that make erratic the network response. This paper focuses on exploring the impact of these buffers management policies on the performance of current interconnection networks, showing a 90\% of performance drop if an incorrect buffers management policy is used. Moreover, this study not only characterizes some of these undesirable scenarios but also proposes practicable solutions.

==> dgfly_drawer.tex <==

%% dgfly drawer
\makeatletter
\newcommand{\dgflydraw}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.9*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={densely dotted,draw,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=.5*\groupnodewidth},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.4*\groupnodewidth},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\begin{scope}[transform shape,rotate=\gangle*\ig]
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,0) node[router](router\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\pgfmathparse{int(\a-2)}
		\let\PPa=\pgfmathresult
		\foreach \ia in {0,...,\PPa}
		{
			\pgfmathparse{int(\ia+1)}
			\let\sia=\pgfmathresult
			\foreach \ja in {\sia,...,\Pa}
			{
				\draw[link] (router\ig_\ia) edge[out=-90,in=-90] (router\ig_\ja);
			}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\pgfmathparse{90+(\ig+.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\aangle=\pgfmathresult
					%\pgfmathparse{90+\resultb*\gangle}
					\pgfmathparse{90+(\resultb-.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\bangle=\pgfmathresult
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[out=\aangle,in=\bangle] (router\resultb_\resulta);
				}{}
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}


\newcommand{\dgflyplusdraw}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.9*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={densely dotted,draw,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=\groupnodewidth},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.2*\groupnodewidth},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\begin{scope}[transform shape,rotate=\gangle*\ig]
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,.3*\groupnodewidth) node[router](router\ig_\ia) {};
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,-.3*\groupnodewidth) node[router](leaf\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\pgfmathparse{90+(\ig+.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\aangle=\pgfmathresult
					%\pgfmathparse{90+\resultb*\gangle}
					\pgfmathparse{90+(\resultb-.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\bangle=\pgfmathresult
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[out=\aangle,in=\bangle] (router\resultb_\resulta);
				}{}
			}
			\foreach \ja in {0,...,\Pa}
			{
				\draw[link] (router\ig_\ia) -- (leaf\ig_\ja);
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}


\newcommand{\dgflydrawrect}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	%\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupwidth}{#6}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	\pgfmathsetlengthmacro{\groupnodeheight}{\groupwidth/\b}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.5*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={very thick,,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=\groupnodeheight},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.6*\groupnodeheight},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		%\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\path ++(0,\ig*\groupnodeheight) node[group](group\ig)  {};
		%\begin{scope}[transform shape,rotate=\gangle*\ig]
		\begin{scope}
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,0) node[router](router\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[in=0,out=0,looseness=0.3] (router\resultb_\resulta);
				}{}
			}
		}
	}
	%intragroup links
	\pgfmathparse{int(\a-2)}
	\global\let\PPa=\pgfmathresult
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\PPa}
		{
			\pgfmathparse{int(\ia+1)}
			\global\let\Sia=\pgfmathresult
			\foreach \na in {\Sia,...,\Pa}
			{
				\draw[link,
					] (router\ig_\ia) edge[in=-90,out=-90,looseness=0.3] (router\ig_\na);
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}
\newcommand{\palmtree@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\pgfmathparse{int(\a-\ia-1)}
	\xdef\resulta{\pgfmathresult}
	\pgfmathparse{int(mod(\ig+1+mod(\resulta*\Dg+\ih,\b-1),\b))}
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@palmtree{%
	\global\let\dgflylink=\palmtree@link
}
\newcommand{\tablelink}[3]{%
	\xdef\resulta{\csname linksa#1_#2_#3\endcsname}
	\xdef\resultb{\csname linksb#1_#2_#3\endcsname}
}
\newcommand\dgfly@configuration@random{%
	\global\let\dgflylink=\tablelink
	\foreach \ib in {0,...,\Pb}
	\foreach \ia in {0,...,\Pa}
	\foreach \idg in {0,...,\Pdg}
	{%
		%\typeout{assigned\ib_\ia_\idg:=-1}
		\expandafter\xdef\csname assigned\ib_\ia_\idg\endcsname{-1}%
	}%
	\foreach \xb in {0,...,\PPb}
	{%
	\pgfmathtruncatemacro\Nxb{\xb+1}%
	\foreach \yb in {\Nxb,...,\Pb}
	\foreach \ti in {1,...,\t}
	{%
		\loop%
			\pgfmathrandominteger{\xia}{0}{\Pa}%
			\pgfmathrandominteger{\xidg}{0}{\Pdg}%
			\xdef\xia{\xia}%
			\xdef\xidg{\xidg}%
			\edef\x{\csname assigned\xb_\xia_\xidg\endcsname}%
			\ifnum \x>-1%
			\repeat%
		%\typeout{assigned\xb_\xia_\xidg:=\yb}%
		\expandafter\xdef\csname assigned\xb_\xia_\xidg\endcsname{\yb}%
		\expandafter\xdef\csname bridge_router\xb_\yb\endcsname{\xia}%
		\expandafter\xdef\csname linksb\xb_\xia_\xidg\endcsname{\yb}%XXX%
		%%%%%%%%%%%%%%%%%%%%%%%%%
		\loop%
			\pgfmathrandominteger{\yia}{0}{\Pa}%
			\pgfmathrandominteger{\yidg}{0}{\Pdg}%
			\xdef\yia{\yia}%
			\xdef\yidg{\yidg}%
			\edef\x{\csname assigned\yb_\yia_\yidg\endcsname}%
			\ifnum \x>-1%
			\repeat%
		\expandafter\xdef\csname assigned\yb_\yia_\yidg\endcsname{\xb}%
		\expandafter\xdef\csname bridge_router\yb_\xb\endcsname{\yia}%
		\expandafter\xdef\csname linksb\yb_\yia_\yidg\endcsname{\yb}%XXX%
		%%
		\expandafter\xdef\csname linksa\xb_\xia_\xidg\endcsname{\yia}%
		\expandafter\xdef\csname linksa\yb_\yia_\yidg\endcsname{\xia}%
	}%
	}%
}
\newcommand{\cycles@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\xdef\resulta{\ia}
	\ifnum\ih=1
		\pgfmathparse{int(mod(\ig+\ia+1,\b))}
	\else
		\pgfmathparse{int(mod(\b+\ig-\ia-1,\b))}
	\fi
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@cycles{%
	\ifnum\Dg=2\relax\else\errmessage{This configuration requires global degree 2}\fi
	\global\let\dgflylink=\cycles@link
}
\newcommand{\hamming@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\xdef\resulta{\ia}
	\pgfmathparse{int(mod(\ig+\ih+1,\b))}
	%\ifnum\ih=1
	%	\pgfmathparse{int(mod(\ig+\ia+1,\b))}
	%\else
	%	\pgfmathparse{int(mod(\b+\ig-\ia-1,\b))}
	%\fi
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@hamming{%
	\ifnum\a=\t\relax\else\errmessage{}\fi
	\global\let\dgflylink=\hamming@link
}
\newcommand{\consecutive@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\pgfmathparse{int(\ia*\Dg+\ih)}
	\let\G=\pgfmathresult
	%\typeout{ig=\ig\ ia=\ia\ ih=\ih\ G=\G}
	\ifnum \G<\ig\relax
		\pgfmathparse{int(floor((\ig-1)/\Dg))}
		\xdef\resulta{\pgfmathresult}
		\xdef\resultb{\G}
	\else
		\pgfmathparse{int(floor((\ig)/\Dg))}
		\xdef\resulta{\pgfmathresult}
		\pgfmathparse{int(\G+1)}
		\xdef\resultb{\pgfmathresult}
	\fi
}
\newcommand\dgfly@configuration@consecutive{%
	\global\let\dgflylink=\consecutive@link
}
\makeatother


==> figures/Hamming/2D_Valiants.tex <==

%% -- common pgfplots prelude --
%\newenvironment{experimentfigure}{\begin{figure}[H]\tikzexternalenable}{\tikzexternaldisable\end{figure}}
%\newenvironment{experimentfigure}{\begin{figure*}}{\end{figure*}}
\pgfplotsset{compat=newest}
\makeatletter
%required for fill plus pattern on boxplot
\tikzset{nomorepostaction/.code=\let\tikz@postactions\pgfutil@empty}
\makeatother
\pgfplotsset{minor grid style={dashed,very thin, color=blue!15}}
\pgfplotsset{major grid style={very thin, color=black!30}}
\pgfplotsset{
	automatically generated axis/.style={
		%default: height=207pt, width=240pt. 240:207 ~~ 7:6
		%height=115pt,%may fit 3figures with 1 line caption
		height=105pt,%may fit 3figures with 2 line caption
		width=174pt,
		scaled ticks=false,
		xticklabel style={font=\tiny,/pgf/number format/.cd, fixed,/tikz/.cd},% formattin ticks' labels
		yticklabel style={font=\tiny,/pgf/number format/.cd, fixed,/tikz/.cd},% formattin ticks' labels
		x label style={at={(ticklabel cs:0.5, -5pt)},name={x label},anchor=north,font=\scriptsize},
		y label style={at={(ticklabel cs:0.5, -5pt)},name={y label},anchor=south,font=\scriptsize},
	},
	automatically generated symbolic/.style={
		height=105pt,
		width=500pt,
		xticklabel style={font=\tiny,rotate=90},
		yticklabel style={font=\tiny,/pgf/number format/.cd, fixed,/tikz/.cd},% formattin ticks' labels
		x label style={at={(ticklabel cs:0.5, -5pt)},name={x label},anchor=north,font=\scriptsize},
		y label style={at={(ticklabel cs:0.5, -5pt)},name={y label},anchor=south,font=\scriptsize},
	},
	first kind/.style={
		%The first axis on each line of plots
		%legend style={overlay,at={(0.50,1.05)},anchor=south,font=\scriptsize,fill=none},
		%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize,fill=none},
		%legend style={at={($(axis description cs:0.00,1.01)!(current page.center)!(axis description cs:1.00,1.01)$)},anchor=south,font=\scriptsize,fill=none},
		legend style={font=\scriptsize,fill=none},
		legend columns=3,legend cell align=left,
	},
	posterior kind/.style={
		%Axis following the first on each line of plots
		%legend style={at={(0.50,1.05)},overlay,anchor=south,font=\tiny,fill=none},
		legend style={draw=none},
	},
}
\def\timetickcode{%
	%\pgfkeys{/pgf/fpu}%
	\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
	%\pgfkeys{/pgf/fpu=true}%
	\pgfmathparse{\tick}%
	%\typeout{tick=\tick, math=\pgfmathresult}%
	\edef\tmp{\pgfmathresult}%
	%\pgfmathsetmacro\xseconds{Mod(\tmp,60)}%
	%\pgfkeys{/pgf/fpu=false}%
	%\pgfmathtruncatemacro\xseconds{Mod(\tmp,60)}%
	%\pgfkeys{/pgf/fpu=true}%
	%\typeout{total seconds=\tmp}%
	%\pgfmathparse{\tmp/60}\typeout{tmp/60=\pgfmathresult}%
	%\pgfmathparse{floor(\tmp/60)}\typeout{floor(tmp/60)=\pgfmathresult}%
	%\pgfmathparse{round(\tmp/60)}\typeout{round(tmp/60)=\pgfmathresult}%
	%\pgfmathparse{int(\tmp/60)}\typeout{int(tmp/60)=\pgfmathresult}%
	\pgfmathtruncatemacro\seconds{\tmp-60*floor(\tmp/60)}%
	%\typeout{truncated seconds=\seconds}%
	\pgfmathtruncatemacro\tmp{(\tmp - \seconds)/60}%
	%\typeout{total minutes=\tmp}%
	%\pgfmathtruncatemacro\minutes{Mod(\tmp,60)}%
	\pgfmathtruncatemacro\minutes{\tmp-60*floor(\tmp/60)}%
	%\typeout{truncated minutes=\seconds}%
	\pgfmathtruncatemacro\tmp{(\tmp - \minutes)/60}%
	%\typeout{total hours=\tmp}%
	%\pgfmathtruncatemacro\hours{Mod(\tmp,24)}%
	\pgfmathtruncatemacro\hours{\tmp-24*floor(\tmp/24)}%
	%\typeout{truncated hours=\hours}%
	\pgfmathtruncatemacro\days{(\tmp - \hours)/24}%
	%{\tiny\days-\hours:\minutes:\seconds}%
	\ifnum\days=0%
		{\tiny\hours:\minutes:\seconds}%
	\else%
		{\tiny\days-\hours:\minutes}%
	\fi%
	%{\tiny\tick}%
}
\def\memorytickcode{%
	\pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
	%\pgfmathprintnumber[sci,sci zerofill,precision=1]{\tick}%
	\pgfmathtruncatemacro\unitcase{log2(\tick+0.001)/10+1.1}%We add a byte to keep the log2 sensible.
	%\pgfmathfloatifflags{}
	\pgfmathparse{\tick / pow(1024,\unitcase-1)}%
	\pgfmathprintnumber{\pgfmathresult}%
	\ifcase\unitcase B%0
		\or KB%1
		\or MB%2
		\or GB%3
		\or TB%4
		\else +1024,\pgfmathprintnumber{unitcase}B%
	\fi%
}
\tikzset{
	automatically generated plot/.style={
		%/pgfplots/error bars/.cd,error bar style={ultra thick},x dir=both, y dir=both,
		/pgfplots/error bars/x dir=both,
		/pgfplots/error bars/y dir=both,
		/pgfplots/error bars/x explicit,
		/pgfplots/error bars/y explicit,
		/pgfplots/error bars/error bar style={ultra thin,solid},
		/tikz/mark options={solid},
	},
	automatically generated bar plot/.style={
		/pgfplots/error bars/y dir=both,
		/pgfplots/error bars/y explicit,
	},
	automatically generated boxplot/.style={
		%/pgfplots/boxplot={
		%	box extend=0.1,
		%	every average/.style={/tikz/mark=*},
		%},
	},
	%/pgf/images/aux in dpth=true,
	x time ticks/.style={
		/pgfplots/scaled x ticks=false,
		/pgfplots/xticklabel={\timetickcode},
	},
	y time ticks/.style={
		/pgfplots/scaled y ticks=false,
		/pgfplots/yticklabel={\timetickcode}
	},
	x memory ticks from kilobytes/.style={
		/pgfplots/scaled x ticks=false,
		/pgfplots/xticklabel={\memorytickcode}
	},
	y memory ticks from kilobytes/.style={
		/pgfplots/scaled y ticks=false,
		/pgfplots/yticklabel={\memorytickcode}
	},
}
\bgroup


%% -- experiment-local prelude
\newcommand\captionprologue{X: }
\newcommand\experimenttitle{hyperx-2d-valiant-pruebas/throughput.pdf (all 180 done)}
\newcommand\experimentheader{\tiny hyperx-2d-valiant-pruebas:throughput.pdf (all 180 done)\\pdflatex on \today\\git\_id=heads/alex-dirty-85a09b18578dc359b59d57b06454c75b50f7196e}
\tikzset{xValiantxoverxDORxfirstx/.style={automatically generated plot,red,solid,mark=o}}
\tikzset{xValiantxoverxDORxfirstxbar/.style={automatically generated bar plot,fill=red!20,postaction={pattern=horizontal lines},}}
\tikzset{xValiantxoverxDORxfirstxboxplot/.style={automatically generated boxplot,fill=red!20,every path/.style={postaction={nomorepostaction,pattern=horizontal lines},}}}
\tikzset{xValiantxoverxDORx/.style={automatically generated plot,green,dashed,mark=square}}
\tikzset{xValiantxoverxDORxbar/.style={automatically generated bar plot,fill=green!20,postaction={pattern=grid},}}
\tikzset{xValiantxoverxDORxboxplot/.style={automatically generated boxplot,fill=green!20,every path/.style={postaction={nomorepostaction,pattern=grid},}}}
\tikzset{xValiantxDORxladderxrealx/.style={automatically generated plot,blue,solid,mark=triangle}}
\tikzset{xValiantxDORxladderxrealxbar/.style={automatically generated bar plot,fill=blue!20,postaction={pattern=horizontal lines},}}
\tikzset{xValiantxDORxladderxrealxboxplot/.style={automatically generated boxplot,fill=blue!20,every path/.style={postaction={nomorepostaction,pattern=horizontal lines},}}}
\def\xValiantxoverxDORxtext{Valiant DOR-2phase minB}
\def\xValiantxoverxDORxfirstxtext{Valiant DOR-2phase minA}
\def\xValiantxDORxladderxrealxtext{Valiant DOR ladder}
%% -- henceafter the data


\begin{experimentfigure}%
	%\begin{center}
	\centering%
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxuniformx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxvaliantxpruebas-throughput-xuniformx}%
	\pgfplotslegendfromname{legend-hyperxxRIIdxvaliantxpruebas-throughput-xuniformx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxuniformx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
	\begin{axis}[
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxvaliantxpruebas-throughput-xuniformx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,
		%ymax=1,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={accepted load},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
	]
\addplot[xValiantxoverxDORxfirstx]	coordinates{(0.1,0.0997593) (0.2,0.20001654) (0.3,0.2992152) (0.4,0.40008083) (0.5,0.4079474) +- (0,0.026453825) (0.6,0.39930645) (0.7,0.40274715) (0.8,0.42029) (0.8999999,0.4086158) (1,0.41331574)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
\addplot[xValiantxoverxDORx] coordinates{(0.1,0.09973759) (0.2,0.20034961) (0.3,0.2999885) (0.4,0.40027082) (0.5,0.4397148) (0.6,0.43943572) (0.7,0.44277143) (0.8,0.43413422) (0.8999999,0.43913403) (1,0.440635)};\addlegendentry{\xValiantxoverxDORxtext}
\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,0.09967437) (0.2,0.19964163) (0.3,0.30005637) (0.4,0.38852617) (0.5,0.38889447) (0.6,0.39101425) (0.7,0.389532) (0.8,0.3902028) (0.8999999,0.38978872) (1,0.38944402)};\addlegendentry{\xValiantxDORxladderxrealxtext}
	\end{axis}
	%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}
%	\centering%
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxbasic-delay-selectorxuniformx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxbasic-delay-xuniformx}%
	%\pgfplotslegendfromname{legend-hyperxxRIIdxbasic-delay-xuniformx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxbasic-delay-selectorxuniformx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
		\begin{axis}[
		title=Uniform,
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxbasic-delay-xuniformx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={average message delay},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
		]
\addplot[xValiantxoverxDORx] coordinates{(0.1,28.761904) (0.2,41.775265) (0.3,66.26163) (0.4,138.9839) (0.5,1094.2279) (0.6,1378.0703) (0.7,1485.0819) (0.8,1533.9259) (0.8999999,1547.877) (1,1570.7363)};\addlegendentry{\xValiantxoverxDORxtext}
\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,29.035965) (0.2,43.329544) (0.3,74.015434) (0.4,766.5721) (0.5,1419.5995) (0.6,1555.1787) (0.7,1620.284) (0.8,1649.604) (0.8999999,1664.9398) (1,1673.4136)};\addlegendentry{\xValiantxDORxladderxrealxtext}
\addplot[xValiantxoverxDORxfirstx] coordinates{(0.1,28.762384) (0.2,41.83905) (0.3,66.466286) (0.4,141.54262) (0.5,1124.1504) (0.6,1410.4966) (0.7,1506.0372) (0.8,1565.6744) (0.8999999,1588.8041) (1,1595.7982)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
		\end{axis}
		%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}
	%\begin{center}
	%\centering%
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxbasicxvaliant-jaingeneration-selectorxuniformx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xuniformx}%
	%\pgfplotslegendfromname{legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xuniformx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxbasicxvaliant-jaingeneration-selectorxuniformx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
		\begin{axis}[
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xuniformx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,
		ymax=1,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={Jain index generation},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
		]
		\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,0.9839116) (0.2,0.99213356) (0.3,0.9949196) (0.4,0.9936002) (0.5,0.9825599) (0.6,0.9804515) (0.7,0.97794676) (0.8,0.98011667) (0.8999999,0.9789066) (1,0.9792342)};\addlegendentry{\xValiantxDORxladderxrealxtext}
		\addplot[xValiantxoverxDORxfirstx] coordinates{(0.1,0.98454005) (0.2,0.99238944) (0.3,0.99473315) (0.4,0.9960072) (0.5,0.9845071) +- (0,0.0060211755) (0.6,0.97921634) (0.7,0.9752433) (0.8,0.97788674) (0.8999999,0.97912556) (1,0.97323674)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
		\addplot[xValiantxoverxDORx] coordinates{(0.1,0.98387533) (0.2,0.9923823) (0.3,0.99484104) (0.4,0.9959523) (0.5,0.98423356) +- (0,0.0016885332) (0.6,0.9736209) +- (0,0.0046036784) (0.7,0.9778078) (0.8,0.9749333) (0.8999999,0.9720814) +- (0.000000073000486,0.0059050904) (1,0.97673774) +- (0,0.0018293187)};\addlegendentry{\xValiantxoverxDORxtext}
		\end{axis}
		%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}


	%\end{center}
	%\caption{\captionprologue "uniform"}%
	%\label{fig:PLACEHOLDER}%
%\end{experimentfigure}
%
%\begin{experimentfigure}%
	%\begin{center}
	%\centering%
%
	%\end{center}
	%\caption{\captionprologue "3-shift on x and y (a.k.a. 2-tornado)"}%
%\end{experimentfigure}
%
%\begin{experimentfigure}%
	%\begin{center}
%	\centering%
%	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxRIIDxDCRx-kind0.md5}%
%	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIDxDCRx}%
%	\pgfplotslegendfromname{legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIDxDCRx}\\
%	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxRIIDxDCRx-kind0}%
%	\begin{tikzpicture}[baseline,remember picture]
%	\begin{axis}[
%		title=DCR-2D,
%		automatically generated axis,
%		first kind,,legend to name=legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIDxDCRx,
		%ybar interval=0.6,
%		 ymin=%(ymin)s,
%		 ymax=%(ymax)s,
%		ymin=0,ymax=1,
		%enlargelimits=false,
%		ymajorgrids=true,
%		yminorgrids=true,
%		xmajorgrids=true,
%		mark options=solid,
%		minor y tick num=4,
		 %(xlabel)s%(ylabel)s
%		xlabel={offered load},
%		ylabel={accepted load},
		%legend style={at={(1.05,1.0)},anchor=north west},
		%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		 %(barprop)s
		%every x tick label/.append style={anchor=base,yshift=-7},
%	]
%\addplot[xValiantxoverxDORxfirstx]  coordinates{(0.1,0.09976856) (0.2,0.2001427) (0.3,0.29916552) (0.4,0.4005964) (0.5,0.4287492) (0.6,0.4269513) (0.7,0.42678377) (0.8,0.429124) (0.8999999,0.4213641) (1,0.4242244)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
%\addplot[xValiantxoverxDORx] coordinates{(0.1,0.099605404) (0.2,0.2004313) (0.3,0.3000289) (0.4,0.40030923) (0.5,0.4200603) (0.6,0.3536774) +- (0,0.10105889) (0.7,0.32898638) +- (0,0.15454398) (0.8,0.27788118) +- (0,0.12385448) (0.8999999,0.28139937) +- (0.000000073000486,0.12559018) (1,0.2806891) +- (0,0.12036746)};\addlegendentry{\xValiantxoverxDORxtext}
%\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,0.09989313) (0.2,0.20011084) (0.3,0.2990484) (0.4,0.3735751) (0.5,0.37452498) (0.6,0.37473714) (0.7,0.3675641) (0.8,0.37243977) (0.8999999,0.370043) (1,0.3699998)};\addlegendentry{\xValiantxDORxladderxrealxtext}
%
%	\end{axis}
%	\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
%	\end{tikzpicture}
	%\end{center}
	\centering
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}%
	%\pgfplotslegendfromname{legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxvaliantxpruebas-throughput-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
	\begin{axis}[
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxvaliantxpruebas-throughput-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,ymax=0.5,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={accepted load},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
	]
\addplot[xValiantxoverxDORxfirstx] coordinates{(0.1,0.0997593) (0.2,0.20001654) (0.3,0.2992152) (0.4,0.40008083) (0.5,0.4079474) +- (0,0.026453825) (0.6,0.39930645) (0.7,0.40274715) (0.8,0.42029) (0.8999999,0.4086158) (1,0.41331574)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
\addplot[xValiantxoverxDORx] coordinates{(0.1,0.0996652) (0.2,0.20023529) (0.3,0.3001236) (0.4,0.39997828) (0.5,0.2890718) +- (0,0.10652303) (0.6,0.18924654) +- (0,0.06631043) (0.7,0.37152043) +- (0,0.040502425) (0.8,0.15995418) +- (0,0.0704797) (0.8999999,0.18873954) +- (0.000000073000486,0.096294805) (1,0.16642223) +- (0,0.08631271)};\addlegendentry{\xValiantxoverxDORxtext}
\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,0.09977934) (0.2,0.19993639) (0.3,0.2992755) (0.4,0.36602056) (0.5,0.3649169) (0.6,0.3623953) (0.7,0.3639605) (0.8,0.36658445) (0.8999999,0.36839995) (1,0.36428973)};\addlegendentry{\xValiantxDORxladderxrealxtext}
	\end{axis}
	%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}
%	\centering%
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxbasic-delay-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxbasic-delay-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}%
	%\pgfplotslegendfromname{legend-hyperxxRIIdxbasic-delay-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxbasic-delay-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
		\begin{axis}[
		title=XY-3shift,
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxbasic-delay-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={average message delay},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
		]
		\addplot[xValiantxoverxDORx] coordinates{(0.1,28.606668) (0.2,42.006443) (0.3,67.75769) (0.4,146.81578) (0.5,1405.2262) +- (0,183.45074) (0.6,1572.5737) (0.7,1683.5941) (0.8,2078.096) +- (0,707.6691) (0.8999999,2144.4932) +- (0.000000073000486,626.41766) (1,2184.5715) +- (0,595.925)};\addlegendentry{\xValiantxoverxDORxtext}
		\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,29.035965) (0.2,43.329544) (0.3,74.015434) (0.4,766.5721) (0.5,1419.5995) (0.6,1555.1787) (0.7,1620.284) (0.8,1649.604) (0.8999999,1664.9398) (1,1673.4136)};\addlegendentry{\xValiantxDORxladderxrealxtext}
		\addplot[xValiantxoverxDORxfirstx] coordinates{(0.1,28.762384) (0.2,41.83905) (0.3,66.466286) (0.4,141.54262) (0.5,1124.1504) (0.6,1410.4966) (0.7,1506.0372) (0.8,1565.6744) (0.8999999,1588.8041) (1,1595.7982)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
		\end{axis}
		%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}
%	\centering%
	\tikzpicturedependsonfile{externalized-plots/external-hyperxxRIIdxbasicxvaliant-jaingeneration-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0.md5}%
	\tikzsetnextfilename{externalized-legends/legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}%
	%\pgfplotslegendfromname{legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx}\\
	\tikzsetnextfilename{externalized-plots/external-hyperxxRIIdxbasicxvaliant-jaingeneration-selectorxRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx-kind0}%
	\begin{tikzpicture}[baseline,remember picture]
		\begin{axis}[
		automatically generated axis,
		first kind,,legend to name=legend-hyperxxRIIdxbasicxvaliant-jaingeneration-xRIIIxshiftxonxxxandxyxxaxkxaxxRIIxtornadoxx,
		%%ybar interval=0.6,
		% ymin=%(ymin)s,
		% ymax=%(ymax)s,
		ymin=0,
		ymax=1,%
		%%enlargelimits=false,
		ymajorgrids=true,
		yminorgrids=true,
		xmajorgrids=true,
		mark options=solid,
		minor y tick num=4,
		% %(xlabel)s%(ylabel)s
		xlabel={offered load},
		ylabel={Jain index generation},
		%%legend style={at={(1.05,1.0)},anchor=north west},
		%%legend style={opacity=0.7,at={(0.99,0.99)},anchor=north east},
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=3,transpose legend,legend cell align=left,
		%%legend style={at={(0.00,1.01)},anchor=south west,font=\scriptsize},legend columns=2,legend cell align=left,
		% %(barprop)s
		%%every x tick label/.append style={anchor=base,yshift=-7},
		]
		\addplot[xValiantxDORxladderxrealx] coordinates{(0.1,0.9838755) (0.2,0.9922374) (0.3,0.99500734) (0.4,0.98620194) (0.5,0.9769203) (0.6,0.9738889) (0.7,0.97405386) (0.8,0.9771324) (0.8999999,0.9748216) (1,0.97390693)};\addlegendentry{\xValiantxDORxladderxrealxtext}
		\addplot[xValiantxoverxDORxfirstx] coordinates{(0.1,0.9841915) (0.2,0.9923708) (0.3,0.995022) (0.4,0.9962804) (0.5,0.96963817) +- (0,0.024444537) (0.6,0.9652006) (0.7,0.96332574) +- (0,0.012138186) (0.8,0.9726936) (0.8999999,0.96595865) (1,0.97111315)};\addlegendentry{\xValiantxoverxDORxfirstxtext}
		\addplot[xValiantxoverxDORx] coordinates{(0.1,0.98380584) (0.2,0.9922185) (0.3,0.9948004) (0.4,0.99623275) (0.5,0.9089742) +- (0,0.07829666) (0.6,0.9491686) +- (0,0.024453279) (0.7,0.93538666) +- (0,0.027325371) (0.8,0.74687177) +- (0,0.37772623) (0.8999999,0.83030295) +- (0.000000073000486,0.21336177) (1,0.85165167) +- (0,0.13454515)};\addlegendentry{\xValiantxoverxDORxtext}
		\end{axis}
		%\pgfresetboundingbox\useasboundingbox (y label.north west) (current axis.north east) ($(current axis.outer north west)!(current axis.north east)!(current axis.outer north east)$);
	\end{tikzpicture}
	\caption{Throughput, average latency and Jain index (fairness) on 2DHyperX of $k=10$ with different VC mechanisms over Valiant routing, under different traffic patterns.}
	\label{fig:2D_valiants_2phases_comparison}%
\end{experimentfigure}

\egroup



==> figures/Other/caminos_hamming.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Plot of paths},
x grid style={darkgray176},
xlabel={k},
xmajorgrids,
xmin=0, xmax=20.95,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Ratio paths of D and D-1},
ymajorgrids,
ymin=-0.049875, ymax=1.047375,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 0
1.19191919191919 0.296107440390692
1.38383838383838 0.47780915339123
1.57575757575758 0.597263313609467
1.76767676767677 0.679967346938776
1.95959595959596 0.739584440429376
2.15151515151515 0.783971434239238
2.34343434343434 0.817906510107016
2.53535353535354 0.84443104077713
2.72727272727273 0.865555555555555
2.91919191919192 0.882652267094503
3.11111111111111 0.896683673469388
3.3030303030303 0.908341048733272
3.49494949494949 0.918131243944001
3.68686868686869 0.926432726590355
3.87878787878788 0.93353271484375
4.07070707070707 0.939652359167288
4.26262626262626 0.944964174209924
4.45454545454545 0.94960433152853
4.64646464646465 0.953681474480151
4.83838383838384 0.957283135969596
5.03030303030303 0.960480476121353
5.22222222222222 0.963331824354912
5.41414141414141 0.965885358654489
5.60606060606061 0.9681811541271
5.7979797979798 0.97025276499654
5.98989898989899 0.972128457638156
6.18181818181818 0.973832179930796
6.37373737373737 0.975384329454668
6.56565656565656 0.976802366863905
6.75757575757576 0.978101309095296
6.94949494949495 0.979294128583018
7.14141414141414 0.980392078407679
7.33333333333333 0.981404958677686
7.52525252525253 0.982341335975857
7.71717171717172 0.983208725089773
7.90909090909091 0.984013740256309
8.1010101010101 0.984762221627975
8.29292929292929 0.985459341494063
8.48484848484848 0.986109693877551
8.67676767676768 0.986717370416097
8.86868686868687 0.987286024875338
9.06060606060606 0.987818928199908
9.25252525252525 0.988319015655689
9.44444444444444 0.98878892733564
9.63636363636363 0.989231043075828
9.82828282828283 0.989647512646174
10.020202020202 0.990040281932882
10.2121212121212 0.990411115709393
10.4040404040404 0.99076161749458
10.5959595959596 0.991093246916351
10.7878787878788 0.991407334932458
10.979797979798 0.991705097205495
11.1717171717172 0.991987645883542
11.3636363636364 0.992256
11.5555555555556 0.992511094674556
11.7474747474747 0.99275378927064
11.9393939393939 0.99298487464248
12.1313131313131 0.993205079586051
12.3232323232323 0.993415076592314
12.5151515151515 0.993615486987671
12.7070707070707 0.993806885535119
12.8989898989899 0.993989804559801
13.0909090909091 0.994164737654321
13.2828282828283 0.994332143012043
13.4747474747475 0.994492446430458
13.6666666666667 0.994646044021416
13.8585858585859 0.994793304660473
14.0505050505051 0.994934572203665
14.2424242424242 0.995070167496605
14.4343434343434 0.995200390197846
14.6262626262626 0.995325520435884
14.8181818181818 0.995445820316911
15.010101010101 0.995561535298497
15.2020202020202 0.995672895442655
15.3939393939394 0.995780116560233
15.5858585858586 0.995883401257283
15.7777777777778 0.995982939892878
15.969696969697 0.996078911456852
16.1616161616162 0.996171484375
16.3535353535354 0.99626081724854
16.5454545454545 0.996347059533873
16.7373737373737 0.996430352168103
16.9292929292929 0.996510828145203
17.1212121212121 0.996588613047224
17.3131313131313 0.996663825534516
17.5050505050505 0.99673657779854
17.6969696969697 0.996806975980484
17.8888888888889 0.99687512055862
18.0808080808081 0.996941106707032
18.2727272727273 0.997005024628103
18.4646464646465 0.997066959860952
18.6565656565657 0.99712699356776
18.8484848484848 0.997185202799806
19.040404040404 0.997241660744816
19.2323232323232 0.997296436957136
19.4242424242424 0.997349597572046
19.6161616161616 0.997401205505488
19.8080808080808 0.997451320640298
20 0.9975
};\addlegendentry{n=2}
\addplot [semithick, darkorange25512714]
table {%
1 0
1.19191919191919 0.0259264579143924
1.38383838383838 0.076935372156215
1.57575757575758 0.133505917159763
1.76767676767677 0.188604081632653
1.95959595959596 0.239797002869593
2.15151515151515 0.286451100972029
2.34343434343434 0.328645214030916
2.53535353535354 0.366724337708925
2.72727272727273 0.401111111111111
2.91919191919192 0.432226625639061
3.11111111111111 0.460459183673469
3.3030303030303 0.486154364110765
3.49494949494949 0.509614420795884
3.68686868686869 0.531101519984988
3.87878787878788 0.55084228515625
4.07070707070707 0.569032504356286
4.26262626262626 0.585841512993868
4.45454545454545 0.601416076634735
4.64646464646465 0.615883742911153
4.83838383838384 0.629355694928108
5.03030303030303 0.641929162432864
5.22222222222222 0.653689452240833
5.41414141414141 0.664711656270884
5.60606060606061 0.675062089116143
5.7979797979798 0.684799499811822
5.98989898989899 0.693976095481574
6.18181818181818 0.702638408304498
6.37373737373737 0.710828031876553
6.56565656565656 0.71858224852071
6.75757575757576 0.725934565344165
6.94949494949495 0.732915173742564
7.14141414141414 0.739551344506041
7.33333333333333 0.745867768595041
7.52525252525253 0.751886851943606
7.71717171717172 0.757628971245306
7.90909090909091 0.7631126965253
8.1010101010101 0.768354985354569
8.29292929292929 0.773371352781211
8.48484848484848 0.778176020408163
8.67676767676768 0.782782047511726
8.86868686868687 0.787201446650858
9.06060606060606 0.791445285846914
9.25252525252525 0.795523779104136
9.44444444444444 0.799446366782007
9.63636363636363 0.803221787112852
9.82828282828283 0.806858139974586
10.020202020202 0.810362943873569
10.2121212121212 0.813743186961231
10.4040404040404 0.817005372796682
10.5959595959596 0.820155561472591
10.7878787878788 0.823199406640576
10.979797979798 0.82614218890306
11.1717171717172 0.828988845979026
11.3636363636364 0.831744
11.5555555555556 0.834411982248521
11.7474747474747 0.836996855613281
11.9393939393939 0.83950243500219
12.1313131313131 0.841932305926022
12.3232323232323 0.844289841440473
12.5151515151515 0.846578217612814
12.7070707070707 0.84880042766043
12.8989898989899 0.850959294892039
13.0909090909091 0.853057484567901
13.2828282828283 0.855097514782634
13.4747474747475 0.857081766463095
13.6666666666667 0.85901249256395
13.8585858585859 0.860891826534862
14.0505050505051 0.862721790125594
14.2424242424242 0.864504300588502
14.4343434343434 0.866241177331895
14.6262626262626 0.867934148072403
14.8181818181818 0.869584854529715
15.010101010101 0.871194857702849
15.2020202020202 0.872765642763325
15.3939393939394 0.874298623597247
15.5858585858586 0.875795147025284
15.7777777777778 0.87725649672684
15.969696969697 0.878683896892294
16.1616161616162 0.880078515625
16.3535353535354 0.881441468112794
16.5454545454545 0.882773819587006
16.7373737373737 0.884076588085367
16.9292929292929 0.885350747033794
17.1212121212121 0.886597227660741
17.3131313131313 0.887816921256615
17.5050505050505 0.889010681289746
17.6969696969697 0.890179325389379
17.8888888888889 0.891323637205355
18.0808080808081 0.892444368153304
18.2727272727273 0.893542239053489
18.4646464646465 0.894617941670776
18.6565656565657 0.895672140162613
18.8484848484848 0.896705472441352
19.040404040404 0.897718551456775
19.2323232323232 0.898711966404209
19.4242424242424 0.899686283863211
19.6161616161616 0.900642048871443
19.8080808080808 0.901579785937978
20 0.9025
};\addlegendentry{n=3}
\addplot [semithick, forestgreen4416044]
table {%
1 0
1.19191919191919 0.00417459915570725
1.38383838383838 0.0213397382623078
1.57575757575758 0.0487810081929904
1.76767676767677 0.0819080583090379
1.95959595959596 0.117426367384594
2.15151515151515 0.153311856858269
2.34343434343434 0.188404368388413
2.53535353535354 0.222080077018951
2.72727272727273 0.254037037037037
2.91919191919192 0.284162833465126
3.11111111111111 0.31245444606414
3.3030303030303 0.338970015343286
3.49494949494949 0.363799889990125
3.68686868686869 0.387049326893169
3.87878787878788 0.408828258514404
4.07070707070707 0.42924536308762
4.26262626262626 0.448404759945544
4.45454545454545 0.466404304328979
4.64646464646465 0.483334850415057
4.83838383838384 0.499280092009772
5.03030303030303 0.514316738575728
5.22222222222222 0.528514876279822
5.41414141414141 0.541938421250702
5.60606060606061 0.554645608354885
5.7979797979798 0.566689481551595
5.98989898989899 0.578118366219051
6.18181818181818 0.588976312843477
6.37373737373737 0.599303507065493
6.56565656565656 0.609136644515248
6.75757575757576 0.618509270921038
6.94949494949495 0.627452089148794
7.14141414141414 0.635993235445082
7.33333333333333 0.64415852742299
7.52525252525253 0.651971686383315
7.71717171717172 0.659454536489697
7.90909090909091 0.666627183171527
8.1010101010101 0.673508172947957
8.29292929292929 0.680114636672392
8.48484848484848 0.686462418002915
8.67676767676768 0.692566188718174
8.86868686868687 0.698439552324622
9.06060606060606 0.704095137241737
9.25252525252525 0.70954468070751
9.44444444444444 0.714799104416853
9.63636363636363 0.71986858278982
9.82828282828283 0.724762604663708
10.020202020202 0.729490029111993
10.2121212121212 0.734059136012505
10.4040404040404 0.738477671916224
10.5959595959596 0.742752891705397
10.7878787878788 0.746891596474455
10.979797979798 0.750900168018605
11.1717171717172 0.754784600272043
11.3636363636364 0.758550528
11.5555555555556 0.762203253015476
11.7474747474747 0.765747768162108
11.9393939393939 0.769188779278656
12.1313131313131 0.772530725337615
12.3232323232323 0.775777796930139
12.5151515151515 0.778933953251499
12.7070707070707 0.782002937725308
12.8989898989899 0.78498829239062
13.0909090909091 0.787893371163409
13.2828282828283 0.790721352072763
13.4747474747475 0.793475248562161
13.6666666666667 0.79615791993732
13.8585858585859 0.798772081034169
14.0505050505051 0.801320311173449
14.2424242424242 0.803805062462075
14.4343434343434 0.806228667495745
14.6262626262626 0.808593346512204
14.8181818181818 0.81090121403998
15.010101010101 0.813154285083345
15.2020202020202 0.815354480880555
15.3939393939394 0.81750363426908
15.5858585858586 0.8196034946886
15.7777777777778 0.821655732849787
15.969696969697 0.823661945094485
16.1616161616162 0.825623657470703
16.3535353535354 0.827542329543822
16.5454545454545 0.829419357963616
16.7373737373737 0.831256079805071
16.9292929292929 0.833053775699459
17.1212121212121 0.834813672770822
17.3131313131313 0.836536947391735
17.5050505050505 0.838224727771174
17.6969696969697 0.839878096386212
17.8888888888889 0.841498092268409
18.0808080808081 0.843085713154881
18.2727272727273 0.844641917513248
18.4646464646465 0.846167626449
18.6565656565657 0.847663725503112
18.8484848484848 0.849131066347196
19.040404040404 0.850570468382918
19.2323232323232 0.851982720251889
19.4242424242424 0.853368581261829
19.6161616161616 0.85472878273433
19.8080808080808 0.856064029279202
20 0.857375
};\addlegendentry{n=4}
\addplot {\x};
\end{axis}

\end{tikzpicture}

